Rewriting XPath Queries using View Intersections: Tractability versus Completeness

The standard approach for optimization of XPath queries by rewriting using views techniques consists in navigating inside a view's output, thus allowing the usage of only one view in the rewritten query. Algorithms for richer classes of XPath rewritings, using intersection or joins on node identifiers, have been proposed, but they either lack completeness guarantees, or require additional information about the data. We identify the tightest restrictions under which an XPath can be rewritten in polynomial time using an intersection of views and propose an algorithm that works for any documents or type of identifiers. As a side-effect, we analyze the complexity of the related problem of deciding if an XPath with intersection can be equivalently rewritten as one without intersection or union. We extend our formal study of the view-based rewriting problem for XPath by describing also (i) algorithms for more complex rewrite plans, with no limitations on the number of intersection and navigation steps inside view outputs they employ, and (ii) adaptations of our techniques to deal with XML documents without persistent node Ids, in the presence of XML keys. Complementing our computational complexity study, we describe a proof-of-concept implementation of our techniques and possible choices that may speed up execution in practice, regarding how rewrite plans are built, tested and executed. We also give a thorough experimental evaluation of these techniques, focusing on scalability and the running time improvements achieved by the execution of view-based plans.

==> abstract-tcs.tex <==
\vspace{-0.05cm}
The standard approach for optimization of XPath queries by rewriting
using views techniques consists in navigating inside a view's output,
thus allowing the usage of only one view in the rewritten query.
Algorithms for richer classes of XPath rewritings, using intersection
or joins on node identifiers, have been proposed, but they either lack
completeness guarantees, or require additional information about the
data. We identify the tightest restrictions under which an XPath can
be rewritten in polynomial time using an intersection of views and
propose an algorithm that works for any documents or type of
identifiers.  As an additional contribution, we analyze the complexity
of the related problem of deciding if an XPath with intersection can
be equivalently rewritten as one without intersection or union.


